Bandit Quickest Changepoint Detection

Many industrial and security applications employ a suite of sensors for detecting abrupt changes in temporal behavior patterns. These abrupt changes typically manifest locally, rendering only a small subset of sensors informative. Continuous monitoring of every sensor can be expensive due to resource constraints, and serves as a motivation for the bandit quickest changepoint detection problem, where sensing actions (or sensors) are sequentially chosen, and only measurements corresponding to chosen actions are observed. We derive an information-theoretic lower bound on the detection delay for a general class of finitely parameterized probability distributions. We then propose a computationally efficient online sensing scheme, which seamlessly balances the need for exploration of different sensing options with exploitation of querying informative actions. We derive expected delay bounds for the proposed scheme and show that these bounds match our information-theoretic lower bounds at low false alarm rates, establishing optimality of the proposed method. We then perform a number of experiments on synthetic and real datasets demonstrating the effectiveness of our proposed method.

==> intro.tex <==
We propose a framework for bandit quickest changepoint detection (BQCD), motivated by real-world applications such as sensor network based surveillance systems~\cite{SSNsurveill}, edge computing in IoT devices~\cite{Aminikhanghahi}, fault monitoring in large-scale industrial systems~\cite{purohit2019}. %, and in general, where real-time anomaly detection in multivariate time-series data is of interest. 
Our goal is to identify changes in behavior of the system state, which evolves over a multi-dimensional space. The state can exhibit abrupt temporal changes, which may manifest in only a few components and be difficult to detect. In surveillance applications, due to narrow receptive fields of sensors (such as cameras), a large number of sensors are required to ensure continuous coverage, and intrusions (abrupt changes) manifest only among a few sensors in the field-of-view. % among all the multi-sensor observations. 
Due to resource constraints  such as limited battery power on edge-devices, sensing, processing and communication may be expensive \cite{halgamuge2009estimation}, and it is desirable to minimize sensor activity at any time. 
%Sensing systems deploying edge-devices are resource constrained, which put hard limits on sensing, processing, computation and communication~\cite{}. As such, at any time, only a few sensors can be queried resulting in bandit information, namely that we only have access to measurements from the queried sensors. %it is impractical to monitor or continuously transmit information from all sensors, and 

%\noindent {\bf Sensing Dilemma.} %These two aspects, namely, local abrupt changes observable only through well-aligned sensing actions together with limits on  monitoring due to cost of sensing actions poses significant challenges. 
%Our conundrum is that monitoring all state components is practically infeasible -- only a few may be accessed at a time. However,  without knowing in advance which component to monitor, local abrupt changes may go undetected.% in real-time. 

\noindent {\bf Bandit Quickest Changepoint Detection (BQCD).}
%We propose a general framework for online changepoint detection with bandit information. In our framework, 
We consider a setting with a finite collection of  sensing actions ${\cal A}$. At any time, $t$, a sensing action $A_t \in {\cal A}$ at time $t$ can be deployed, and we obtain a measurement $X_t$ in response (the `bandit' setting\footnote{Our usage follows classical multi-armed bandits terminology, where bandits refers to the fact that actions can yield only partial information \cite{lattimore2020bandit}.}). The measurement $X_t$ follows a probability law, $\mathbb{P}_t[\cdot \mid A_t, \nu]$, that depends both on the sensing action chosen as well as the time $\nu$ when abrupt change occurs, and is otherwise independent of past history. The probability laws before and after the change belong to a finitely parameterized family of distributions $\mathbb{P}_t[\cdot \mid A_t,\nu]\triangleq \Pobs{\theta_{\nu, t}}{\cdot}{A_t}$. %  \mathbb{P}(\cdot \mid a_t,\theta_{\nu,t}), \,\,\theta_{\nu,t} \in \Theta$. 
%
Our objective is to sequentially choose sensing actions so as to minimize the detection delay from when a change has occurred, while keeping false detection behavior of abrupt change below a pre-specified level\footnote{For a trivial action set ($|\mathcal{A}| = 1$), this is the classical quickest change detection problem where the only adaptive decision is whether to stop or not, see e.g., \cite{tartakovsky2014sequential}}.  

{\bf Regret vs. Detection Delay Metric.} The performance measure we adopt is not the usual regret or shortfall in cumulative `reward' but detection delay instead, where each time spent after the real changepoint `costs' one unit of loss. This is similar to the sample complexity metric in inference-based bandit tasks like best arm identification or bandit hypothesis testing \cite{garivier-kaufmann16optimal-best-arm-fixed-confidence}, but having the added complexity of handling  non-stationary distributional change with a false alarm rate constraint.

\noindent {\bf Information-theoretic Lower Bound.} We prove a lower bound on the expected detection delay that any BQCD algorithm must suffer at a fixed false alarm rate. The lower bound exhibits a fundamental tradeoff between early stopping (false-alarm) and detection delay (time to detect abrupt change). It offers the key insight that the quickest way to detect a change, at any false-alarm rate, is by playing the `most informative action', of an `oracle' who a priori knows the post-change distribution. This suggests that to quickly identify changepoints, we must direct our effort towards rapidly identifying informative actions. On a technical level, we develop a change-of-measure argument for nonstationary, adaptive change detection, that allows for relating the divergences between random trajectories until stopping to the divergence of probability laws under each action for any two problem instances.

%To prove this bound, we appeal to an information inequality due to \cite{garivier-kaufmann16optimal-best-arm-fixed-confidence}, a now standard change-of-measure tool for establishing fundamental limits on learning procedures. In our context, this inequality allows us to examine divergences between the laws of random trajectories until detection with a more convenient quantity corresponding to early stopping.   

\noindent{\bf $\epsilon$-Greedy Change Detector (\egcd).} We propose \egcd, which, at a high level, uses a small amount of forced exploration to identify informative actions. The forced exploration allows for rapid convergence towards informative actions, and playing these actions minimizes detection delay. Our \egcd\, is based on the generalized max-likelihood/likelihood ratio principle which is utilized to estimate parametric changes. To prove detection delay bounds we draw upon key insights of \egcd. We first interpret the scheme in terms of competing parallel `queues', where each queue corresponds to a candidate post-change parameter, collects `arrivals' which are log-likelihood ratios of observations, and cannot go negative. The true parameter is the queue which enjoys the highest growth rate after a change, and the detection delay is the time required for it to dominate and become the `longest queue'. The dynamics of the queues can be related to nonstationary random walks with drifts. Using these insights, we prove that the expected detection delay of \egcd\, at low false alarm rates mirrors our information theoretic lower bounds thus establishing optimality of our method.
%For Gaussian distributions, we utilize the intuition that the dynamics of the queues corresponds to random walks with the true parameter corresponding to one with maximum drift.
\if0
We provide several interpretations of our method to develop key insights, including one where the true change parameter corresponds to the `longest queue' in queueing system, and as a random walk associated with the maximum drift, where each . 

Alternatively, we can interpret our algorithm from the perspective of competing random walks, where each random walk corresponds to a 

In particular, the Gaussian family of distributions lends to the perspective that we have multiple competing random walks, with each random walk corresponding to a different parameter in the Gaussian family, and the random walk associated with the true distribution has the maximum drift. As such, our analysis is based on characterizing the minimum time required for the ground-truth random walk to dominate its competitors. 
We find that our analysis leads us to conclude that for suitable families of finitely parameterized distributions, and for sufficiently small false alarm rates, the expected delay matches our information theoretic lower bound upto constants. As such our analysis demonstrates the optimality of the proposed \egcd \, scheme.\fi 

\noindent {\bf Experiments.} We perform numerical experiments of \egcd\, on synthetic and real datasets and show that under variations of changepoints, anomalies, and action sets, we realize gains due to adaptivity. 
%Synthetic experiments are performed on line and grid graphs to illustrate \egcd\, under different conditions such as varying actions sets, locality of anomalies, and changepoints. Under these varying conditions, \egcd\, exhibits detection delays that is close to oracle delays. As such, purely random action choices perform poorly, pointing to the gains due to adaptivity. We also perform experiments on an industrial machine sensing problem, where the cost arises due to the fact that high-fidelity degradation detection for individual machines requires significant processing. We show that \egcd\, performance is comparable to that of an oracle. 

%from processing required for high-fidelity. In this problem sensing actions have different costs because they require different levels of computation, and the goal is to choose low-cost sensing actions when possible without sacrificing performance. Our results again show that \egcd\, performance is close to Oracle performance.

%Another example involves industrial sensing systems, which utilize multi-modal sensors of varying degrees of fidelity. Here anomalies can go undetected if measurements from a suitable sensor are not observed.  
